Cellular Load Dependent Sleep Control for Energy Efficient HetNets with Non-Uniform User Distributions

This study proposes a novel stochastic geometry framework analyzing power control strategies in spatially correlated network topologies. Heterogeneous networks are studied, with users modeled via the superposition of homogeneous and Poisson cluster processes. First, a new expression approaching the distribution of the number of users per base station is provided. This distribution defines the load associated with each Vorono\"i cell, capturing non-uniformities in user locations and correlation to BSs positions. The power allocation is adjusted based on this load, allowing BSs to enter sleep mode when their activity falls below a defined threshold. Furthermore, the propagation model features millimeter wave transmission characteristics and directional beamforming. Considering these aspects, revisited definitions of coverage probability, spectral efficiency, and energy efficiency are proposed. Tractable expressions for these metrics are derived and validated using Monte-Carlo simulations. Asymptotic expressions are also proposed, providing further understanding on the influence of the system parameters. Our numerical results finally analyze the impact of the sleep control on the performance and display the optimal strategies in terms of energy efficiency.

==> Text/Tikz.tex <==


\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,405); %set diagram left start at 0, and has height of 405
{
\small\fontfamily{ptm}\selectfont
%Rounded Rect [id:dp20336162232913035] 
\draw  [fill={rgb, 255:red, 248; green, 231; blue, 28 }  ,fill opacity=0.2 ] (220.5,24.85) .. controls (220.5,17.2) and (226.7,11) .. (234.35,11) -- (424.65,11) .. controls (432.3,11) and (438.5,17.2) .. (438.5,24.85) -- (438.5,66.4) .. controls (438.5,74.05) and (432.3,80.25) .. (424.65,80.25) -- (234.35,80.25) .. controls (226.7,80.25) and (220.5,74.05) .. (220.5,66.4) -- cycle ;
%Straight Lines [id:da5699287830092794] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ] [dash pattern={on 0.84pt off 2.51pt}]  (140,52.25) -- (230.5,52.25) ;
\draw [shift={(233.5,52.25)}, rotate = 180] [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (10.72,-5.15) -- (0,0) -- (10.72,5.15) -- (7.12,0) -- cycle    ;
%Rounded Rect [id:dp21831812529156225] 
\draw  [fill={rgb, 255:red, 126; green, 211; blue, 33 }  ,fill opacity=0.2 ] (30.5,140.85) .. controls (30.5,116.49) and (50.24,96.75) .. (74.6,96.75) -- (206.9,96.75) .. controls (231.26,96.75) and (251,116.49) .. (251,140.85) -- (251,337.15) .. controls (251,361.51) and (231.26,381.25) .. (206.9,381.25) -- (74.6,381.25) .. controls (50.24,381.25) and (30.5,361.51) .. (30.5,337.15) -- cycle ;
%Straight Lines [id:da9353838689314125] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ] [dash pattern={on 0.84pt off 2.51pt}]  (140,52.25) -- (140.5,110.25) ;
%Straight Lines [id:da6080929724308939] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ] [dash pattern={on 0.84pt off 2.51pt}]  (140.5,179.75) -- (140.5,162.75) ;
\draw [shift={(140.5,159.75)}, rotate = 90] [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (10.72,-5.15) -- (0,0) -- (10.72,5.15) -- (7.12,0) -- cycle    ;
%Straight Lines [id:da19885502981491054] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ] [dash pattern={on 0.84pt off 2.51pt}]  (90.5,205.25) -- (109.5,205.25) ;
\draw [shift={(112.5,205.25)}, rotate = 180] [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (10.72,-5.15) -- (0,0) -- (10.72,5.15) -- (7.12,0) -- cycle    ;
%Shape: Ellipse [id:dp3441672320860596] 
\draw  [fill={rgb, 255:red, 255; green, 255; blue, 255 }  ,fill opacity=1 ] (122,267.88) .. controls (122,257.31) and (130.84,248.75) .. (141.75,248.75) .. controls (152.66,248.75) and (161.5,257.31) .. (161.5,267.88) .. controls (161.5,278.44) and (152.66,287) .. (141.75,287) .. controls (130.84,287) and (122,278.44) .. (122,267.88) -- cycle ;

%Straight Lines [id:da9200895982226993] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ] [dash pattern={on 0.84pt off 2.51pt}]  (164.5,268) -- (183,268.75) ;
\draw [shift={(161.5,267.88)}, rotate = 2.33] [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (10.72,-5.15) -- (0,0) -- (10.72,5.15) -- (7.12,0) -- cycle    ;
%Straight Lines [id:da040347827386499446] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ] [dash pattern={on 0.84pt off 2.51pt}]  (141.25,248.75) -- (141.25,231.75) ;
\draw [shift={(141.25,228.75)}, rotate = 90] [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (10.72,-5.15) -- (0,0) -- (10.72,5.15) -- (7.12,0) -- cycle    ;
%Straight Lines [id:da026073273837253108] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ] [dash pattern={on 0.84pt off 2.51pt}]  (99.5,267.75) -- (119,267.86) ;
\draw [shift={(122,267.88)}, rotate = 180.32] [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (10.72,-5.15) -- (0,0) -- (10.72,5.15) -- (7.12,0) -- cycle    ;
%Straight Lines [id:da575691635885293] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ] [dash pattern={on 0.84pt off 2.51pt}]  (141.75,307) -- (141.75,290) ;
\draw [shift={(141.75,287)}, rotate = 90] [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (10.72,-5.15) -- (0,0) -- (10.72,5.15) -- (7.12,0) -- cycle    ;
%Rounded Rect [id:dp626319075457844] 
\draw  [fill={rgb, 255:red, 74; green, 144; blue, 226 }  ,fill opacity=0.2 ] (409.5,141.1) .. controls (409.5,116.74) and (429.24,97) .. (453.6,97) -- (585.9,97) .. controls (610.26,97) and (630,116.74) .. (630,141.1) -- (630,337.15) .. controls (630,361.51) and (610.26,381.25) .. (585.9,381.25) -- (453.6,381.25) .. controls (429.24,381.25) and (409.5,361.51) .. (409.5,337.15) -- cycle ;
%Straight Lines [id:da8504974353842569] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ] [dash pattern={on 0.84pt off 2.51pt}]  (430,53.22) -- (520.5,52.25) ;
\draw [shift={(427,53.25)}, rotate = 359.39] [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (10.72,-5.15) -- (0,0) -- (10.72,5.15) -- (7.12,0) -- cycle    ;
%Straight Lines [id:da048574116903484565] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ] [dash pattern={on 0.84pt off 2.51pt}]  (520.5,52.25) -- (521,125.25) ;
%Straight Lines [id:da43567394879215504] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ] [dash pattern={on 0.84pt off 2.51pt}]  (483.5,123.75) -- (553,123.75) ;
%Straight Lines [id:da867025181544437] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ] [dash pattern={on 0.84pt off 2.51pt}]  (581.5,190.75) -- (581.27,161) ;
\draw [shift={(581.25,158)}, rotate = 89.56] [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (10.72,-5.15) -- (0,0) -- (10.72,5.15) -- (7.12,0) -- cycle    ;
%Straight Lines [id:da8613024862600447] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ] [dash pattern={on 0.84pt off 2.51pt}]  (460.5,191.75) -- (460.27,162) ;
\draw [shift={(460.25,159)}, rotate = 89.56] [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (10.72,-5.15) -- (0,0) -- (10.72,5.15) -- (7.12,0) -- cycle    ;
%Straight Lines [id:da5040107845698154] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ] [dash pattern={on 0.84pt off 2.51pt}]  (461,273.25) -- (460.77,243.5) ;
\draw [shift={(460.75,240.5)}, rotate = 89.56] [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (10.72,-5.15) -- (0,0) -- (10.72,5.15) -- (7.12,0) -- cycle    ;
%Rounded Rect [id:dp7080347935080331] 
\draw  [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=0.2 ] (260.88,196.47) .. controls (260.88,181.11) and (273.32,168.67) .. (288.68,168.67) -- (372.08,168.67) .. controls (387.43,168.67) and (399.88,181.11) .. (399.88,196.47) -- (399.88,353.53) .. controls (399.88,368.89) and (387.43,381.33) .. (372.08,381.33) -- (288.68,381.33) .. controls (273.32,381.33) and (260.88,368.89) .. (260.88,353.53) -- cycle ;
%Straight Lines [id:da4233378300261248] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ] [dash pattern={on 0.84pt off 2.51pt}]  (330.02,80.75) -- (331,212.75) ;
\draw [shift={(330,77.75)}, rotate = 89.58] [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (10.72,-5.15) -- (0,0) -- (10.72,5.15) -- (7.12,0) -- cycle    ;
%Straight Lines [id:da7800462403483797] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ] [dash pattern={on 0.84pt off 2.51pt}]  (487,144.75) -- (552,145.23) ;
\draw [shift={(555,145.25)}, rotate = 180.42] [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (10.72,-5.15) -- (0,0) -- (10.72,5.15) -- (7.12,0) -- cycle    ;
%Straight Lines [id:da582702196876097] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ] [dash pattern={on 0.84pt off 2.51pt}]  (330.83,271.42) -- (330.61,241.67) ;
\draw [shift={(330.58,238.67)}, rotate = 89.56] [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (10.72,-5.15) -- (0,0) -- (10.72,5.15) -- (7.12,0) -- cycle    ;
%Shape: Rectangle [id:dp5723923367113168] 
\draw  [fill={rgb, 255:red, 255; green, 255; blue, 255 }  ,fill opacity=1 ] (234,29.83) -- (425.5,29.83) -- (425.5,74.5) -- (234,74.5) -- cycle ;

% Text Node
\draw (244.67,33.33) node [anchor=north west, align=center][inner sep=0.75pt]{Performance metric AAKCP\\ eq. \eqref{eq:AAKCP_gen}};
% Text Node
\draw (292,12.5) node [anchor=north west][inner sep=0.75pt]   [align=left] {{\small {\fontfamily{ptm}\selectfont Section III.A}}};
% Text Node
\draw (140,58) node [anchor=north west][inner sep=0.75pt]   [align=left] {{\small {\fontfamily{ptm}\selectfont Section III.B}}};
% Text Node
\draw  [fill={rgb, 255:red, 255; green, 255; blue, 255 }  ,fill opacity=1 ]  (113.5,111.5) -- (168.5,111.5) -- (168.5,158.5) -- (113.5,158.5) -- cycle  ;
\draw (116.5,115.5) node [anchor=north west][inner sep=0.75pt]   [align=left] {\begin{minipage}[lt]{34.36pt}\setlength\topsep{0pt}
\begin{center}
{\small $p_{\mathcal{A}_{k,i}}(a)$}\\{\small eq. \eqref{eq:pmf_act}}
\end{center}

\end{minipage}};
% Text Node
\draw  [fill={rgb, 255:red, 255; green, 255; blue, 255 }  ,fill opacity=1 ]  (113,181.5) -- (168,181.5) -- (168,228.5) -- (113,228.5) -- cycle  ;
\draw (116,185.5) node [anchor=north west][inner sep=0.75pt]   [align=left] {\begin{minipage}[lt]{34.36pt}\setlength\topsep{0pt}
\begin{center}
{\small $\displaystyle G_{S}$}\\{\small eq. \eqref{eq:PGF_S}}
\end{center}

\end{minipage}};
% Text Node
\draw  [fill={rgb, 255:red, 255; green, 255; blue, 255 }  ,fill opacity=1 ]  (39.5,181) -- (88.5,181) -- (88.5,228) -- (39.5,228) -- cycle  ;
\draw (42.5,185) node [anchor=north west][inner sep=0.75pt]   [align=left] {\begin{minipage}[lt]{30.79pt}\setlength\topsep{0pt}
\begin{center}
{\small $\displaystyle f_{R_c}$}\\{\small Lem. 1}
\end{center}

\end{minipage}};
% Text Node
\draw (141.54,267.3) node[inner sep=0.75pt]{$\prod $};
% Text Node
\draw  [fill={rgb, 255:red, 255; green, 255; blue, 255 }  ,fill opacity=1 ]  (35.5,245.5) -- (98.5,245.5) -- (98.5,292.5) -- (35.5,292.5) -- cycle  ;
\draw (38.5,249.5) node [anchor=north west][inner sep=0.75pt]   [align=left] {\begin{minipage}[lt]{40.05pt}\setlength\topsep{0pt}
\begin{center}
{\scriptsize $\displaystyle \forall u \in \mathcal{K}_{1/2}^\textup{UE}$}\\{\small Lem. 2}
\end{center}

\end{minipage}};
% Text Node
\draw  [fill={rgb, 255:red, 255; green, 255; blue, 255 }  ,fill opacity=1 ]  (183,245) -- (246,245) -- (246,292) -- (183,292) -- cycle  ;
\draw (186,249) node [anchor=north west][inner sep=0.75pt]   [align=left] {\begin{minipage}[lt]{40.05pt}\setlength\topsep{0pt}
\begin{center}
{\scriptsize $\displaystyle \forall u \in \mathcal{K}_{3}^\textup{UE}$}\\{\small Lem. 4}
\end{center}

\end{minipage}};
% Text Node
\draw  [fill={rgb, 255:red, 255; green, 255; blue, 255 }  ,fill opacity=1 ]  (111.5,308.5) -- (168.5,308.5) -- (168.5,355.5) -- (111.5,355.5) -- cycle  ;
\draw (114.5,312.5) node [anchor=north west][inner sep=0.75pt]   [align=left] {\begin{minipage}[lt]{35.89pt}\setlength\topsep{0pt}
\begin{center}
{\scriptsize $\displaystyle \Phi _{d,0}^\textup{UE}$}\\{\small  Lem. 3 }
\end{center}

\end{minipage}};
% Text Node
\draw (69.5,358.33) node [anchor=north west][inner sep=0.75pt]   [align=left] {{\small Modelling of the activity}};
% Text Node
\draw (441.5,58) node [anchor=north west][inner sep=0.75pt]   [align=left] {{\small {\fontfamily{ptm}\selectfont Section III.D}}};
% Text Node
\draw  [fill={rgb, 255:red, 255; green, 255; blue, 255 }  ,fill opacity=1 ]  (555,111) -- (609,111) -- (609,158) -- (555,158) -- cycle  ;
\draw (558,115) node [anchor=north west][inner sep=0.75pt]   [align=left] {\begin{minipage}[lt]{33.97pt}\setlength\topsep{0pt}
\begin{center}
{\small $\displaystyle \mathbb{P}_\text{cov}$}\\{\small  \ Th. 3 } 
\end{center}

\end{minipage}};
% Text Node
\draw  [fill={rgb, 255:red, 255; green, 255; blue, 255 }  ,fill opacity=1 ]  (435,110.5) -- (486,110.5) -- (486,157.5) -- (435,157.5) -- cycle  ;
\draw (438,114.5) node [anchor=north west, align=center][inner sep=0.75pt] {\small $\mathbb{P}_\text{suc}$\\ Th. 1-2};

% Text Node
\draw  [fill={rgb, 255:red, 255; green, 255; blue, 255 }  ,fill opacity=1 ]  (549,191.5) -- (614,191.5) -- (614,239.5) -- (549,239.5) -- cycle  ;
\draw (552,195.5) node [anchor=north west][inner sep=0.75pt]   [align=left] {\begin{minipage}[lt]{41.57pt}\setlength\topsep{0pt}
\begin{center}
{\small $\displaystyle \mathbb{P}( S_{\Phi _{j}})$}\\{\small  \ Lem. 9} \ 
\end{center}
\end{minipage}};
% Text Node
\draw  [fill={rgb, 255:red, 255; green, 255; blue, 255 }  ,fill opacity=1 ]  (428.5,191) -- (493.5,191) -- (493.5,240) -- (428.5,240) -- cycle  ;
\draw (431.5,195) node [anchor=north west][inner sep=0.75pt]   [align=left] {\begin{minipage}[lt]{41.57pt}\setlength\topsep{0pt}
\begin{center}
{\small $\displaystyle \mathcal{L}_{\mathcal{I}}^\text{tot}$}\\{\small  \ Lem. 8} \ 
\end{center}

\end{minipage}};
% Text Node
\draw  [fill={rgb, 255:red, 255; green, 255; blue, 255 }  ,fill opacity=1 ]  (428.5,274.5) -- (493.5,274.5) -- (493.5,325.5) -- (428.5,325.5) -- cycle  ;
\draw (431.5,278.5) node [anchor=north west][inner sep=0.75pt]   [align=left] {\begin{minipage}[lt]{41.57pt}\setlength\topsep{0pt}
\begin{center}
{\small $\displaystyle \mathcal{L}_{g_{\mathbf{x}_k}}$}\\{\small  \ Lem. 7} \ 
\end{center}

\end{minipage}};
% Text Node
\draw (438.5,357) node [anchor=north west][inner sep=0.75pt]   [align=left] {{\small Coverage \& success prob.}};
% Text Node
\draw (269,354.6) node [anchor=north west][inner sep=0.75pt]   [align=left] {{\small Distance distribution}};
% Text Node
\draw (251,121.67) node [anchor=north west][inner sep=0.75pt]   [align=left] {{\small {\fontfamily{ptm}\selectfont Section III.C}}};
% Text Node
\draw  [fill={rgb, 255:red, 255; green, 255; blue, 255 }  ,fill opacity=1 ]  (306.67,191.33) -- (355.67,191.33) -- (355.67,238.33) -- (306.67,238.33) -- cycle  ;
\draw (309.67,195.33) node [anchor=north west, align=center][inner sep=0.75pt] {\small $\mathbb{P}_\text{closest}$\\ Lem. 6};

% Text Node
\draw  [fill={rgb, 255:red, 255; green, 255; blue, 255 }  ,fill opacity=1 ]  (299,274.17) -- (364,274.17) -- (364,322.17) -- (299,322.17) -- cycle  ;
\draw (302,278.17) node [anchor=north west, align=center][inner sep=0.75pt] {\small $f_{R_{j,i}} | F_{R_{j,i}}$\\ Lem. 5};
}


\end{tikzpicture}


==> Text/Tikz2.tex <==



\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,405); %set diagram left start at 0, and has height of 405

%Rounded Rect [id:dp20336162232913035] 
\draw  [fill={rgb, 255:red, 248; green, 231; blue, 28 }  ,fill opacity=0.2 ] (220.5,24.85) .. controls (220.5,17.2) and (226.7,11) .. (234.35,11) -- (424.65,11) .. controls (432.3,11) and (438.5,17.2) .. (438.5,24.85) -- (438.5,66.4) .. controls (438.5,74.05) and (432.3,80.25) .. (424.65,80.25) -- (234.35,80.25) .. controls (226.7,80.25) and (220.5,74.05) .. (220.5,66.4) -- cycle ;
%Straight Lines [id:da5699287830092794] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ] [dash pattern={on 0.84pt off 2.51pt}]  (140,52.25) -- (230.5,52.25) ;
\draw [shift={(233.5,52.25)}, rotate = 180] [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (10.72,-5.15) -- (0,0) -- (10.72,5.15) -- (7.12,0) -- cycle    ;
%Rounded Rect [id:dp21831812529156225] 
\draw  [fill={rgb, 255:red, 126; green, 211; blue, 33 }  ,fill opacity=0.2 ] (30.5,140.85) .. controls (30.5,116.49) and (50.24,96.75) .. (74.6,96.75) -- (206.9,96.75) .. controls (231.26,96.75) and (251,116.49) .. (251,140.85) -- (251,337.15) .. controls (251,361.51) and (231.26,381.25) .. (206.9,381.25) -- (74.6,381.25) .. controls (50.24,381.25) and (30.5,361.51) .. (30.5,337.15) -- cycle ;
%Straight Lines [id:da9353838689314125] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ] [dash pattern={on 0.84pt off 2.51pt}]  (140,52.25) -- (140.5,110.25) ;
%Straight Lines [id:da6080929724308939] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ] [dash pattern={on 0.84pt off 2.51pt}]  (140.5,179.75) -- (140.5,162.75) ;
\draw [shift={(140.5,159.75)}, rotate = 90] [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (10.72,-5.15) -- (0,0) -- (10.72,5.15) -- (7.12,0) -- cycle    ;
%Straight Lines [id:da19885502981491054] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ] [dash pattern={on 0.84pt off 2.51pt}]  (90.5,205.25) -- (109.5,205.25) ;
\draw [shift={(112.5,205.25)}, rotate = 180] [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (10.72,-5.15) -- (0,0) -- (10.72,5.15) -- (7.12,0) -- cycle    ;
%Shape: Ellipse [id:dp3441672320860596] 
\draw  [fill={rgb, 255:red, 255; green, 255; blue, 255 }  ,fill opacity=1 ] (122,267.88) .. controls (122,257.31) and (130.84,248.75) .. (141.75,248.75) .. controls (152.66,248.75) and (161.5,257.31) .. (161.5,267.88) .. controls (161.5,278.44) and (152.66,287) .. (141.75,287) .. controls (130.84,287) and (122,278.44) .. (122,267.88) -- cycle ;

%Straight Lines [id:da9200895982226993] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ] [dash pattern={on 0.84pt off 2.51pt}]  (164.5,268) -- (183,268.75) ;
\draw [shift={(161.5,267.88)}, rotate = 2.33] [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (10.72,-5.15) -- (0,0) -- (10.72,5.15) -- (7.12,0) -- cycle    ;
%Straight Lines [id:da040347827386499446] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ] [dash pattern={on 0.84pt off 2.51pt}]  (141.25,248.75) -- (141.25,231.75) ;
\draw [shift={(141.25,228.75)}, rotate = 90] [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (10.72,-5.15) -- (0,0) -- (10.72,5.15) -- (7.12,0) -- cycle    ;
%Straight Lines [id:da026073273837253108] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ] [dash pattern={on 0.84pt off 2.51pt}]  (99.5,267.75) -- (119,267.86) ;
\draw [shift={(122,267.88)}, rotate = 180.32] [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (10.72,-5.15) -- (0,0) -- (10.72,5.15) -- (7.12,0) -- cycle    ;
%Straight Lines [id:da575691635885293] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ] [dash pattern={on 0.84pt off 2.51pt}]  (141.75,307) -- (141.75,290) ;
\draw [shift={(141.75,287)}, rotate = 90] [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (10.72,-5.15) -- (0,0) -- (10.72,5.15) -- (7.12,0) -- cycle    ;
%Rounded Rect [id:dp626319075457844] 
\draw  [fill={rgb, 255:red, 74; green, 144; blue, 226 }  ,fill opacity=0.2 ] (409.5,141.1) .. controls (409.5,116.74) and (429.24,97) .. (453.6,97) -- (585.9,97) .. controls (610.26,97) and (630,116.74) .. (630,141.1) -- (630,337.15) .. controls (630,361.51) and (610.26,381.25) .. (585.9,381.25) -- (453.6,381.25) .. controls (429.24,381.25) and (409.5,361.51) .. (409.5,337.15) -- cycle ;
%Straight Lines [id:da8504974353842569] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ] [dash pattern={on 0.84pt off 2.51pt}]  (430,53.22) -- (520.5,52.25) ;
\draw [shift={(427,53.25)}, rotate = 359.39] [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (10.72,-5.15) -- (0,0) -- (10.72,5.15) -- (7.12,0) -- cycle    ;
%Straight Lines [id:da048574116903484565] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ] [dash pattern={on 0.84pt off 2.51pt}]  (520.5,52.25) -- (521,125.25) ;
%Straight Lines [id:da43567394879215504] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ] [dash pattern={on 0.84pt off 2.51pt}]  (483.5,123.75) -- (553,123.75) ;
%Straight Lines [id:da867025181544437] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ] [dash pattern={on 0.84pt off 2.51pt}]  (581.5,190.75) -- (581.27,161) ;
\draw [shift={(581.25,158)}, rotate = 89.56] [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (10.72,-5.15) -- (0,0) -- (10.72,5.15) -- (7.12,0) -- cycle    ;
%Straight Lines [id:da8613024862600447] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ] [dash pattern={on 0.84pt off 2.51pt}]  (460.5,191.75) -- (460.27,162) ;
\draw [shift={(460.25,159)}, rotate = 89.56] [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (10.72,-5.15) -- (0,0) -- (10.72,5.15) -- (7.12,0) -- cycle    ;
%Rounded Rect [id:dp7080347935080331] 
\draw  [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=0.2 ] (260.88,196.47) .. controls (260.88,181.11) and (273.32,168.67) .. (288.68,168.67) -- (372.08,168.67) .. controls (387.43,168.67) and (399.88,181.11) .. (399.88,196.47) -- (399.88,353.53) .. controls (399.88,368.89) and (387.43,381.33) .. (372.08,381.33) -- (288.68,381.33) .. controls (273.32,381.33) and (260.88,368.89) .. (260.88,353.53) -- cycle ;
%Straight Lines [id:da4233378300261248] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ] [dash pattern={on 0.84pt off 2.51pt}]  (330.02,80.75) -- (331,212.75) ;
\draw [shift={(330,77.75)}, rotate = 89.58] [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (10.72,-5.15) -- (0,0) -- (10.72,5.15) -- (7.12,0) -- cycle    ;
%Straight Lines [id:da7800462403483797] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ] [dash pattern={on 0.84pt off 2.51pt}]  (487,144.75) -- (552,145.23) ;
\draw [shift={(555,145.25)}, rotate = 180.42] [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (10.72,-5.15) -- (0,0) -- (10.72,5.15) -- (7.12,0) -- cycle    ;
%Straight Lines [id:da582702196876097] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ] [dash pattern={on 0.84pt off 2.51pt}]  (330.83,271.42) -- (330.61,241.67) ;
\draw [shift={(330.58,238.67)}, rotate = 89.56] [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (10.72,-5.15) -- (0,0) -- (10.72,5.15) -- (7.12,0) -- cycle    ;
%Shape: Rectangle [id:dp5723923367113168] 
\draw  [fill={rgb, 255:red, 255; green, 255; blue, 255 }  ,fill opacity=1 ] (234,29.83) -- (425.5,29.83) -- (425.5,74.5) -- (234,74.5) -- cycle ;
%Rounded Rect [id:dp5501198104158489] 
\draw  [fill={rgb, 255:red, 74; green, 144; blue, 226 }  ,fill opacity=0.2 ] (421.5,271.6) .. controls (421.5,262.76) and (428.66,255.6) .. (437.5,255.6) -- (607,255.6) .. controls (615.84,255.6) and (623,262.76) .. (623,271.6) -- (623,319.6) .. controls (623,328.44) and (615.84,335.6) .. (607,335.6) -- (437.5,335.6) .. controls (428.66,335.6) and (421.5,328.44) .. (421.5,319.6) -- cycle ;
%Straight Lines [id:da6688767724963327] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ] [dash pattern={on 0.84pt off 2.51pt}]  (522,254.6) -- (521,125.25) ;

% Text Node
\draw (242.67,30.33) node [anchor=north west][inner sep=0.75pt]   [align=left] {\begin{minipage}[lt]{115.95pt}\setlength\topsep{0pt}
\begin{center}
{\small Performance metric AAKCP}\\{\small eq. (11)}
\end{center}

\end{minipage}};
% Text Node
\draw (290,9.5) node [anchor=north west][inner sep=0.75pt]   [align=left] {{\small {\fontfamily{ptm}\selectfont Section 3.A}}};
% Text Node
\draw (144,55) node [anchor=north west][inner sep=0.75pt]   [align=left] {{\small {\fontfamily{ptm}\selectfont Section 3.B}}};
% Text Node
\draw  [fill={rgb, 255:red, 255; green, 255; blue, 255 }  ,fill opacity=1 ]  (113.5,111.5) -- (167.5,111.5) -- (167.5,157.5) -- (113.5,157.5) -- cycle  ;
\draw (114.5,112.5) node [anchor=north west][inner sep=0.75pt]   [align=left] {\begin{minipage}[lt]{34.35pt}\setlength\topsep{0pt}
\begin{center}
{\small $\displaystyle p_{\mathcal{A}}( n)$}\\{\small eq. (15)}
\end{center}

\end{minipage}};
% Text Node
\draw  [fill={rgb, 255:red, 255; green, 255; blue, 255 }  ,fill opacity=1 ]  (113,181.5) -- (167,181.5) -- (167,227.5) -- (113,227.5) -- cycle  ;
\draw (114,182.5) node [anchor=north west][inner sep=0.75pt]   [align=left] {\begin{minipage}[lt]{34.35pt}\setlength\topsep{0pt}
\begin{center}
{\small $\displaystyle G_{S}$}\\{\small eq. (14)}
\end{center}

\end{minipage}};
% Text Node
\draw  [fill={rgb, 255:red, 255; green, 255; blue, 255 }  ,fill opacity=1 ]  (39.5,181) -- (88.5,181) -- (88.5,227) -- (39.5,227) -- cycle  ;
\draw (40.5,182) node [anchor=north west][inner sep=0.75pt]   [align=left] {\begin{minipage}[lt]{30.78pt}\setlength\topsep{0pt}
\begin{center}
{\small $\displaystyle f_{R}{}_{c}$}\\{\small Lem. 1}
\end{center}

\end{minipage}};
% Text Node
\draw  [fill={rgb, 255:red, 255; green, 255; blue, 255 }  ,fill opacity=1 ]  (35.5,245.5) -- (98.5,245.5) -- (98.5,291.5) -- (35.5,291.5) -- cycle  ;
\draw (36.5,246.5) node [anchor=north west][inner sep=0.75pt]   [align=left] {\begin{minipage}[lt]{40.07pt}\setlength\topsep{0pt}
\begin{center}
{\scriptsize $\displaystyle \forall u\ \in \mathcal{E}_{1/2}^{UE}$}\\{\small Lem. 2}
\end{center}

\end{minipage}};
% Text Node
\draw  [fill={rgb, 255:red, 255; green, 255; blue, 255 }  ,fill opacity=1 ]  (183,245) -- (246,245) -- (246,291) -- (183,291) -- cycle  ;
\draw (184,246) node [anchor=north west][inner sep=0.75pt]   [align=left] {\begin{minipage}[lt]{40.07pt}\setlength\topsep{0pt}
\begin{center}
{\scriptsize $\displaystyle \forall u\ \in \mathcal{E}_{3}^{UE}$}\\{\small Lem. 4}
\end{center}

\end{minipage}};
% Text Node
\draw  [fill={rgb, 255:red, 255; green, 255; blue, 255 }  ,fill opacity=1 ]  (111.5,308.5) -- (167.5,308.5) -- (167.5,354.5) -- (111.5,354.5) -- cycle  ;
\draw (112.5,309.5) node [anchor=north west][inner sep=0.75pt]   [align=left] {\begin{minipage}[lt]{35.88pt}\setlength\topsep{0pt}
\begin{center}
{\scriptsize $\displaystyle \Phi _{d,0}^{UE}$}\\{\small  Lem. 3 }
\end{center}

\end{minipage}};
% Text Node
\draw (67.5,355.33) node [anchor=north west][inner sep=0.75pt]   [align=left] {{\small Modelling of the activity}};
% Text Node
\draw (440.5,55) node [anchor=north west][inner sep=0.75pt]   [align=left] {{\small {\fontfamily{ptm}\selectfont Section 3.D}}};
% Text Node
\draw  [fill={rgb, 255:red, 255; green, 255; blue, 255 }  ,fill opacity=1 ]  (555,111) -- (609,111) -- (609,157) -- (555,157) -- cycle  ;
\draw (556,112) node [anchor=north west][inner sep=0.75pt]   [align=left] {\begin{minipage}[lt]{33.96pt}\setlength\topsep{0pt}
\begin{center}
{\small $\displaystyle \mathbb{P}_{cov}$}\\{\small  \ Th. 3 } 
\end{center}

\end{minipage}};
% Text Node
\draw  [fill={rgb, 255:red, 255; green, 255; blue, 255 }  ,fill opacity=1 ]  (435,110.5) -- (485,110.5) -- (485,156.5) -- (435,156.5) -- cycle  ;
\draw (436,111.5) node [anchor=north west][inner sep=0.75pt]   [align=left] {\begin{minipage}[lt]{31.8pt}\setlength\topsep{0pt}
\begin{center}
{\small $\displaystyle \mathbb{P}_{suc}$}\\{\small Th. 1-2}
\end{center}

\end{minipage}};
% Text Node
\draw  [fill={rgb, 255:red, 255; green, 255; blue, 255 }  ,fill opacity=1 ]  (549,191.5) -- (614,191.5) -- (614,238.5) -- (549,238.5) -- cycle  ;
\draw (550,192.5) node [anchor=north west][inner sep=0.75pt]   [align=left] {\begin{minipage}[lt]{41.55pt}\setlength\topsep{0pt}
\begin{center}
{\small $\displaystyle \mathbb{P}( S_{\Phi _{j}})$}\\{\small  \ Lem. 8} \ 
\end{center}

\end{minipage}};
% Text Node
\draw  [fill={rgb, 255:red, 255; green, 255; blue, 255 }  ,fill opacity=1 ]  (428.5,191) -- (493.5,191) -- (493.5,239) -- (428.5,239) -- cycle  ;
\draw (429.5,192) node [anchor=north west][inner sep=0.75pt]   [align=left] {\begin{minipage}[lt]{41.55pt}\setlength\topsep{0pt}
\begin{center}
{\small $\displaystyle \mathcal{L}_{I}^{tot}$}\\{\small  \ Lem. 7} \ 
\end{center}

\end{minipage}};
% Text Node
\draw (436.5,354) node [anchor=north west][inner sep=0.75pt]   [align=left] {{\small Coverage \& success prob.}};
% Text Node
\draw (267,351.6) node [anchor=north west][inner sep=0.75pt]   [align=left] {{\small Distance distribution}};
% Text Node
\draw (258,118.67) node [anchor=north west][inner sep=0.75pt]   [align=left] {{\small {\fontfamily{ptm}\selectfont Section 3.C}}};
% Text Node
\draw  [fill={rgb, 255:red, 255; green, 255; blue, 255 }  ,fill opacity=1 ]  (306.67,191.33) -- (355.67,191.33) -- (355.67,237.33) -- (306.67,237.33) -- cycle  ;
\draw (307.67,192.33) node [anchor=north west][inner sep=0.75pt]   [align=left] {\begin{minipage}[lt]{30.78pt}\setlength\topsep{0pt}
\begin{center}
{\small $\displaystyle \mathbb{P}_{closest}$}\\{\small Lem. 6}
\end{center}

\end{minipage}};
% Text Node
\draw  [fill={rgb, 255:red, 255; green, 255; blue, 255 }  ,fill opacity=1 ]  (299,274.17) -- (364,274.17) -- (364,321.17) -- (299,321.17) -- cycle  ;
\draw (300,275.17) node [anchor=north west][inner sep=0.75pt]   [align=left] {\begin{minipage}[lt]{41.5pt}\setlength\topsep{0pt}
\begin{center}
{\small $\displaystyle f_{R_{j,i}} |\ F_{R_{j,i}}$}\\{\small Lem. 5}
\end{center}

\end{minipage}};
% Text Node
\draw (439.5,264) node [anchor=north west][inner sep=0.75pt]   [align=left] {Asymptotic \\expressions};
% Text Node
\draw (444.5,305) node [anchor=north west][inner sep=0.75pt]   [align=left] {{\small {\fontfamily{ptm}\selectfont Section 3.E}}};
% Text Node
\draw  [fill={rgb, 255:red, 255; green, 255; blue, 255 }  ,fill opacity=1 ]  (556,273) -- (610,273) -- (610,319) -- (556,319) -- cycle  ;
\draw (557,274) node [anchor=north west][inner sep=0.75pt]   [align=left] {\begin{minipage}[lt]{33.96pt}\setlength\topsep{0pt}
\begin{center}
{\small $\displaystyle \mathbb{P}_{suc}$}\\{\small  \ Th. 4 } 
\end{center}

\end{minipage}};
% Text Node
\draw (125.54,243.9) node [anchor=north west][inner sep=0.75pt]    {$\prod $};


\end{tikzpicture}
